Algebraic proof theory for LE-logics

In this paper we extend the research programme in algebraic proof theory from axiomatic extensions of the full Lambek calculus to logics algebraically captured by certain varieties of normal lattice expansions (normal LE-logics). Specifically, we generalise the residuated frames in [34] to arbitrary signatures of normal lattice expansions (LE). Such a generalization provides a valuable tool for proving important properties of LE-logics in full uniformity. We prove semantic cut elimination for the display calculi D.LE associated with the basic normal LE-logics and their axiomatic extensions with analytic inductive axioms. We also prove the finite model property (FMP) for each such calculus D.LE, as well as for its extensions with analytic structural rules satisfying certain additional properties.

==> ProperDisplayCalculiForBasicNormalLE-logics.tex <==
\subsection{Proper display calculi for basic normal LE-logics} \label{ssec:syntactic frames associated w algebras}
\marginnote{AP: I simplified the presentation as discussed. the calculus $\mathrm{D.LE}^\ast$ is a simple instantiation, and I'm not sure that we actually need it at all? }

In this section we  recall the definition of %and define the display calculus $\mathrm{D.LE^\ast}$ for the fully residuated normal $\bbL^\ast_{LE}$ generated by the basic normal $\mathcal{L}_{LE}$-logic and and its cut-free counterpart $\mathrm{cfD.LE^\ast}$. 
the proper display calculus $\mathrm{D.LE}$ for the basic normal $\mathcal{L}$-logic and and its cut-free counterpart $\mathrm{cfD.LE}$ for a fixed but arbitrary LE-signature $\mathcal{L} = \mathcal{L}(\mathcal{F}, \mathcal{G})$  (cf.~Section \ref{subset:language:algsemantics}.1). %\footnote{If $\mathcal{L}$ is fully residuated, then  the corresponding proper display calculus $\mathrm{D.LE}^\ast$ is defined verbatim.} 
Our presentation is a more streamlined version of the one introduced in \cite{greco2018unified} for DLE-logics and then straightforwardly generalized to LE-logics in \cite{ChnGrePalTzi21}. % is obtained from $\mathrm{D.LE^\ast}$ by deleting the logical (also called operational) rules for the operators that do not occur in the original LE-signature. As is usual of existing logical systems covered by the present framework  (e.g.~intuitionistic and bi-intuitionistic logics, or modal and tense logics \cite{gore1998substructural}),\marginnote{here we need to refer to all the examples mentioned above and also to frameworks which are not covered by Gor\'e} the languages manipulated by these calculi are built up using {\em one and the same} set of structural terms, and differ only in the set of operational (also called logical) term constructors.

Let $S_{\mathcal{F}}: = \{\FH \mid f\in \mathcal{F}^*\}$ and $S_{\mathcal{G}}: = \{\GC \mid g\in \mathcal{G}^*\}$ be the sets of structural connectives associated with  $\mathcal{F}^*$ and $ \mathcal{G}^*$ respectively, where $\mathcal{L}(\mathcal{F}^*, \mathcal{G}^\ast)$ denotes the fully residuated language-expansion of $\mathcal{L}(\mathcal{F}, \mathcal{G})$. Each such structural connective has the same arity and  order-type  of its associated  $f\in \mathcal{F}^\ast$ (resp.~$g\in \mathcal{G}^\ast$).\marginnote{AP: I commented the itemization because it is redundant; we have already said everything we needed to say in the previous paragraph and people can go to the appendix to check where a certain residual belongs}
\iffalse
\begin{itemize}
\item Structural symbols for any $f\in \mathcal{F}$ and $g\in \mathcal{G}$: 
%			\begin{center}
%				\begin{tabular}{|r|c|c|c|c|}
%					\hline
%					\scriptsize{Structural symbols} & \mc{2}{c|}{$H$} & \mc{2}{c|}{$K$} \\
%					\hline
%					\scriptsize{Operational symbols} & $f$ & $\phantom{f}$ & $\phantom{g}$ & $g$ \\
%					\hline
%				\end{tabular}
%			\end{center}
%
			\begin{center}
				\begin{tabular}{|r|c|c|}
					\hline
					\scriptsize{Structural symbols} & $\rule{0pt}{2.25ex}\hat{f}$ & $\check{g}$ \\
					\hline
					\scriptsize{Operational symbols} & $f$ & $g$ \\
					\hline
				\end{tabular}
			\end{center}
			
			\item Structural symbols for any $f_i^\sharp, g_h^\flat \in (\mathcal{F}^*\cup \mathcal{G}^*)\setminus (\mathcal{F}\cup \mathcal{G})$, and any $0\leq i\leq n_f$ and $0\leq h\leq n_g$:
%			\begin{center}
%				\begin{tabular}{|r|c|c|c|c|c|c|c|c|}
%					\hline
%					\scriptsize{Structural symbols} & \mc{2}{c|}{$H_i$ ($\varepsilon_f(i) = 1$)} & \mc{2}{c|}{$H_i$ ($\varepsilon_f(i) = \partial$)} & \mc{2}{c|}{$K_h$ ($\varepsilon_g(h) = 1$)} & \mc{2}{c|}{$K_h$ ($\varepsilon_g(h) = \partial$)} \\
%					\hline
%					\scriptsize{Operational symbols} & \ \ \ \ \ \ \ \, & $ (f_i^\sharp)$ & \,\,$(f_i^\sharp)\,\, $ &  & \ \,$(g_h^\flat)$\ \, & $\phantom{(g_h^\flat)}$ & $\phantom{(g_h^\flat)}$ \ \,& \,$(g_h^\flat)\,$\\
%					\hline
%				\end{tabular}
%			\end{center}
\begin{center}
\begin{tabular}{|r|c|c|c|c|}
\hline
\scriptsize{Order type}              & $\varepsilon_{f,i} = \partial$ & $\varepsilon_{f,j} = 1$ & $\varepsilon_{g,h} = 1$ & $\varepsilon_{g,k} = \partial$ \\
\hline
\scriptsize{Structural symbols} & $\FHS_i$                              & $\rule[-1.2ex]{0pt}{0ex}\FCS_j\rule{0pt}{2.5ex}$                                    & $\GHF_h$                             & $\GCF_k$                                       \\
\hline
\scriptsize{Operational symbols} & $(f_i^\sharp)$ & $\rule[-1.2ex]{0pt}{0ex}(f_j^\sharp)\rule{0pt}{2.5ex}$ & $(g_h^\flat)$ & $(g_k^\flat)$ \\
\hline
\end{tabular}
\end{center}

\end{itemize}
The operational symbols which appear above in parentheses do so as a reminder that, unlike their associated structural symbols, might occur only in the language and in the calculus for $\bbL_\mathrm{LE}^*$.
\fi
 

 %Now, given the sets $\mathsf{Str}_\mathcal F$, $\mathsf{Str}_\mathcal G$ defined below and any order type $\epsilon$ on $n$, we let $\mathsf{Str}_\mathcal{F}^{\epsilon} : = \prod_{i = 1}^{n}\mathsf{Str}_{\mathcal{F}^{\epsilon_i}}$ and $\mathsf{Str}_\mathcal{G}^{\epsilon} : = \prod_{i = 1}^{n}\mathsf{Str}_{\mathcal{G}^{\epsilon_i}}$. 

%, where for all $1 \leq i \leq n$,
%
%\begin{center}
%\begin{tabular}{ll}
%$\mathsf{Str}_\mathcal{F}^{\epsilon(i)} = \begin{cases} 
%\mathsf{Str}_\mathcal{F} &\mbox{ if } \epsilon(i) = 1\\
%\mathsf{Str}_\mathcal{G} &\mbox{ if } \epsilon(i) = \partial
%\end{cases}\quad$
%&
%$\mathsf{Str}_\mathcal{G}^{\epsilon(i)} = \begin{cases}
%\mathsf{Str}_\mathcal{G}& \mbox{ if } \epsilon(i) = 1,\\
%\mathsf{Str}_\mathcal{F} & \mbox{ if } \epsilon(i) = \partial.
%\end{cases}$
%\end{tabular}
%\end{center}
\begin{comment}
For notational convenience, we let   $\mathcal F^\partial: =\mathcal G$ and 
$\mathcal G^\partial:=\mathcal F$.\marginnote{AP: where do we use this notation?} Also, for simplicity of presentation, we will sometimes   group together all positive coordinates and all negative coordinates of connectives in vectors, and write e.g.~$k (\ophi, \opsi)$ for $k \in \mathcal{F}^* \cup \mathcal{G}^*$, where  $\ophi$ (resp.~$\opsi$) is the vector of all formulas occurring in the positive (resp.~negative) coordinates of $k$, so that we can dispense with mentioning the order types of coordinates; likewise, we will write $K (\overline{\Sigma}, \overline{\Pi})$ where $K \in S_{\mathcal{F}} \cup S_{\mathcal{G}}$   and $\overline{\Sigma}$ (resp.~$\overline{\Pi}$) is the vector of all structures  occurring in the positive (resp.~negative) coordinates of $K$.
\end{comment}

The calculus $\mathrm{D.LE}$ manipulates sequents $\Gamma \Rightarrow \Delta$, where % both formulas and 
$\Gamma$ and $\Delta$ are structures of two sorts which are built from formulas and are defined by the following simultaneous recursions: 

\begin{center}
\begin{tabular}{@{}r@{}l@{}}
$\rule[-1.2ex]{0pt}{0ex}\mathsf{Fm} \ni \varphi$ \ & $::=\ p \mid \bot \mid \top \mid  \varphi \vee \varphi \mid \varphi \wedge \varphi \mid f (\ophi) \mid g (\ophi) %\mid \fs (\ophi, \opsi) \mid \gf (\ophi, \opsi)
$ \\
%$ \\ \rule[-1.2ex]{0pt}{0ex}  & $\phantom{::=\ \,} 

%\rule[-1.2ex]{0pt}{0ex}$\mathsf{AtomStr}_\mathcal{F} \ni \gamma$ \ & $ ::=\  \varphi$  \\
%$\rule[-1.2ex]{0pt}{0ex}\mathsf{AtomStr}_\mathcal{G} \ni \delta$ \ & $ ::=\  \varphi$  \\

\rule[-1.2ex]{0pt}{0ex}$\mathsf{Str}_\mathcal{F} \ni \Gamma$ \ & $ ::=\  \varphi \mid \AATOP \mid \FH\, (\OSI) %\mid \FHS_i\, (\OGA, \ODE) \mid \GHF_h\, (\OGA, \ODE)
$ \\

\rule[-1.2ex]{0pt}{0ex}$\mathsf{Str}_\mathcal{G} \ni \Delta$ \ & $ ::=\  \varphi \mid \ABOT \mid \GC\, (\OSI)$ \\
%\mid \GCF_k\, (\OGA, \ODE) \mid \FCS_j\, (\OGA, \ODE)$ \\
\end{tabular}
\end{center}

\noindent where $p$ is an atomic formula and $f \in \mathcal{F}$ and $g \in \mathcal{G}$ and $\FH %\FHS_i, \GHF_h 
\in S_{\mathcal{F}}$ and $\GC
%, \GCF_j, \FCS_k 
\in S_{\mathcal{G}}$, %$\Gamma^{\partial} \in \mathsf{Str}_\mathcal{G}$, $\Delta^{1} \in \mathsf{Str}_\mathcal{G}$, $\Delta^{\partial} \in \mathsf{Str}_\mathcal{F}$, and $\Sigma \in \{\mathsf{Str}_\mathcal{F} \cup \mathsf{Str}_\mathcal{G}\}$.
and $\overline{\Sigma}\in \mathsf{Str}_\mathcal{F}^{\epsilon_f}$ (resp.~$\overline{\Sigma}\in \mathsf{Str}_\mathcal{G}^{\epsilon_g}$) for any  $\overline{\Sigma}$ in the argument of $\FH$ (resp.~$\overline{\Sigma}$ in the argument of $\GC(\overline{\Sigma})$). Here $\mathsf{Str}_\mathcal{F}^{\epsilon_f}$ is defined as $\mathsf{Str}_\mathcal{F}^{\epsilon_1}\times\cdots\times \mathsf{Str}_\mathcal{F}^{\epsilon_n}$ where $\mathsf{Str}_\mathcal{F}^\partial=\mathsf{Str}_\mathcal{G}$, and dually for $\mathsf{Str}_\mathcal{G}^{\epsilon_g}$.

In what follows, for every $K \in \{S_{\mathcal{F}} \cup S_{\mathcal{G}}\}$ we use $K(\OSI)[\Gamma]_i$ (resp.~$K(\OSI)[\Delta]_i$) to indicate that the structure $\Gamma$ (resp.~$\Delta$) occurs in the $i$-th coordinate of the vector $\OSI$. 

% for all $1 \leq i \leq n_f$,
%\[
%x^{\epsilon_f(i)} \in \begin{cases} 
%\mathsf{Str}_\mathcal{F}&\mbox{ if } \epsilon_f(i) = 1\\
%\mathsf{Str}_\mathcal{G} &\mbox{ if } \epsilon_f(i) = \partial
%\end{cases}
%\] 
%and for all $1 \leq i \leq n_g$,
%\[
%y^{\epsilon_g(i)} \in \begin{cases}
%\mathsf{Str}_\mathcal{G}& \mbox{ if } \epsilon_g(i) = 1,\\
%\mathsf{Str}_\mathcal{F} & \mbox{ if } \epsilon_g(i) = \partial.
%\end{cases}
%\]
%In what follows, we let $\bari{x} := (x_1, \ldots, x_{i-1}, x_{i+1},\ldots, x_n)$ and $\bari{x}_z := (x_1, \ldots, x_{i-1}, z, x_{i+1},\ldots, x_n)$. $\bari{y}$ and $\bari{y}_z$ are defined likewise. 

%In what follows, we use $\Sigma_1, \ldots, \Sigma_n$ as structure metavariables in $\mathsf{Str}_\mathcal{F} \cup \mathsf{Str}_\mathcal{G}$. Notice that $\Sigma \in \mathsf{Str}_\mathcal{F}$ whenever it occurs in precedent position, and $\Sigma \in \mathsf{Str}_\mathcal{G}$ whenever it occurs in succedent position. The calculus $\mathrm{D.L^\ast_{LE}}$ consists of the following rules: for any $f, \fs, \gf \in \mathcal{F}$ and $g, \gf, \fs \in \mathcal{G}$ and $\FH, \FHS, \GHF \in S_{\mathcal{F}}$ and $\GC, \GCF, \FCS \in S_{\mathcal{G}}$,

\begin{itemize}
\item Identity and cut rules:\footnote{Notice that in the display calculi literature, the identity rule is sometimes defined as $\varphi \fCenter \varphi$, where $\varphi$ is an arbitrary, possibly complex, formula. The difference is inessential given that, in any display calculus, $p \fCenter p$ is an instance of $\varphi \fCenter \varphi$, and $\varphi \fCenter \varphi$ is derivable for any formula $\varphi$ whenever $p \fCenter p$ is the Identity rule.}
\end{itemize}
\begin{center}
\begin{tabular}{rl}
\AXC{\phantom{$\Gamma \fCenter \varphi$}}
\LL{\fns Id}
\UI$p \fCenter p$
\DP
 & 
\AX$\Gamma \fCenter \varphi$
\AX$\varphi \fCenter \Delta$
\RL{\fns Cut}
\BI$\Gamma \fCenter \Delta$
\DP
 \\
\end{tabular}
\end{center}

%\item Display rules: 
%$$
%			\begin{array}{cc}
%			\AX$\FH (\overline{x}) \fCenter y$
%			\doubleLine
%			\LL{$(\epsilon_{f,i} = 1)$}
%			\UI$x_i \fCenter \G_{f^\sharp_{i}}(\bari{x}_y)$
%			\DP
%			&
%			\quad
%			\AxiomC{$\Gamma \Rightarrow \GC(\overline{y})$}
%			\doubleLine
%			\RightLabel{$(\epsilon_{g,i} = 1)$}
%			\UnaryInfC{$\F_{g^\flat_{i}}(\bari{y}_x)\Rightarrow y_i$}
%			\DisplayProof
%			\end{array}
%			$$
%			$$
%			\begin{array}{cc}
%			\AxiomC{$\FH(\overline{x}) \Rightarrow y$}
%			\doubleLine
%			\LeftLabel{$(\epsilon_{f,i} = \partial)$}
%			\UnaryInfC{$\F_{f^\sharp_{i}}(\bari{x}_y)\Rightarrow x_i$}
%			\DisplayProof
%			&
%			\quad
%			\AxiomC{$x \Rightarrow \GC(\overline{y})$}
%			\doubleLine
%			\RightLabel{($\epsilon_{g,i} = \partial)$}
%			\UnaryInfC{$y_i \Rightarrow \G_{g^\flat_{i}}(\bari{y}_x)$}
%			\DisplayProof
%			\end{array}
%			$$

\begin{itemize}		
\item Display postulates for $f\in \mathcal{F}$ and $g\in \mathcal{G}$: for any $1\leq i \leq n_f$ and $1\leq j\leq n_g$,
\end{itemize}
\begin{itemize}
\item[] If $\varepsilon_{f,i} = 1$ and $\varepsilon_{g,j} = 1$,\footnote{The notation $\FH \dashv \FCS_i$ (resp.~$\GHF_j \dashv \GC$) indicates that $\FH$ and $\FCS_i$ (resp.~$\GHF_j$ and $\GC$) are in a {\em residuated pair} and $\FCS_i$ (resp.~$\GHF_j$) is the right residual (resp.~left residual) of $\FH$ (resp.~$\GC$) in the $i$-th coordinate (resp.~$j$-th coordinate).}
\end{itemize}
\begin{center}
\begin{tabular}{@{}c@{}c@{}}
\AXC{$\FH\, (\OSI)[\Gamma]_i \fCenter \Delta$}
\doubleLine
\LL{\fns $\FH \dashv \FCS_i$}
\UIC{$\Gamma \fCenter \FCS_i\, (\OSI)[\Delta]_i$}
\DP
 & \quad
\AXC{$\Gamma \fCenter \GC\, (\OSI)[\Delta]_j$}
\doubleLine
\RL{\fns $\GHF_j \dashv \GC$}
\UIC{$\GHF_j\, (\OSI)[\Gamma]_j \fCenter \Delta$}
\DP \\
\end{tabular}
\end{center}

\begin{itemize}
\item[] If $\varepsilon_{f,i} = \partial$ and $\varepsilon_{g,j} = \partial$,\footnote{The notation $(\GC, \GCF_j)$ (resp.~$(\FH, \FHS_i)$) indicates that $\GC$ and $\GCF_j$ (resp.~$\FH$ and $\FHS_i$) are in a {\em Galois connection} (resp.~{\em dual Galois connection}) and $\GCF_j$ (resp.~$\FHS_i$) is the right residual (resp.~left residual) of $\GC$ (resp.~$\FH$) in the $j$-th coordinate (resp.~$i$-th coordinate).}
\end{itemize}
\begin{center}
\begin{tabular}{@{}c@{}c@{}}					
\AX$\FH\, (\OSI)[\Delta]_i \fCenter \Delta'$
\doubleLine
\LL{\fns $(\FH, \FHS_i)$}
\UI$\FHS_i\, (\OSI)[\Delta']_i \fCenter \Delta$
\DP
 & \quad
\AX$\Gamma' \fCenter \GC\, (\OSI)[\Gamma]_j$
\doubleLine
\RL{\fns $(\GC, \GCF_j)$}
\UI$ \Gamma \fCenter \GCF_j\, (\OSI)[\Gamma']_j$
\DP \\
\end{tabular}
\end{center}

\begin{comment}
\begin{itemize}
\item Necessitation for $f\in \mathcal{F}$ and $g\in \mathcal{G}$: for any $1\leq k \leq n_f$ and $1\leq h\leq n_g$,
\end{itemize}

\begin{center}
\begin{tabular}{c}
\bottomAlignProof
\AXC{$\Big(\Gamma_i \vdash \Delta_i \quad \Delta_j \vdash \Gamma_j \mid i \neq k, 1\leq i, j\leq n_f, \varepsilon_f(i) = 1\mbox{ and } \varepsilon_f(j) = \partial \Big) \quad\quad\quad\quad \Gamma_k \vdash \ABOT$}
\LL{$(\varepsilon_f(k) = 1)$}
\UIC{$\Gamma_k \vdash \FCS_k (\Sigma_1,\ldots, \Sigma_{k-1}, \ABOT, \Sigma_{k+1}, \ldots, \Sigma_{n_f})$}
\DP \\
\end{tabular}
\end{center}


\begin{center}
\begin{tabular}{c}
\bottomAlignProof
\AXC{$\Big(\Gamma_i \vdash \Delta_i \quad \Delta_j \vdash \Gamma_j \mid j \neq k, 1\leq i, j\leq n_f, \varepsilon_f(i) = 1\mbox{ and } \varepsilon_f(j) = \partial \Big) \quad\quad\quad\quad \AATOP \vdash \Delta_k$}
\LL{$(\varepsilon_f(k) = \partial)$}
\UIC{$\FHS_k (\Sigma_1,\ldots, \Sigma_{k-1}, \AATOP, \Sigma_{k+1}, \ldots, \Sigma_{n_f}) \vdash \Delta_k$}
\DP \\
\end{tabular}
\end{center}

%%%

\begin{center}
\begin{tabular}{c}
\bottomAlignProof
\AXC{$\Big(\Gamma_j \vdash \Delta_j \quad \Delta_i \vdash \Gamma_i \mid i \neq h, 1\leq i, j\leq n_f, \varepsilon_g(i) = 1\mbox{ and } \varepsilon_g(j) = \partial \Big) \quad\quad\quad\quad \AATOP \vdash \Delta_h$}
\LL{$(\varepsilon_g(h) = 1)$}
\UIC{$\GHF_h (\Sigma_1,\ldots, \Sigma_{h-1}, \AATOP, \Sigma_{h+1}, \ldots, \Sigma_{n_g}) \vdash \Delta_h$}
\DP \\
\end{tabular}
\end{center}


\begin{center}
\begin{tabular}{c}
\bottomAlignProof
\AXC{$\Big(\Gamma_j \vdash \Delta_j \quad \Delta_i \vdash \Gamma_i \mid j \neq h, 1\leq i, j\leq n_f, \varepsilon_g(i) = 1\mbox{ and } \varepsilon_g(j) = \partial \Big) \quad\quad\quad\quad \Gamma_h \vdash \ABOT$}
\LL{$(\varepsilon_g(h) = \partial)$}
\UIC{$\Gamma_h \vdash \GCF_h (\Sigma_1,\ldots, \Sigma_{h-1}, \ABOT, \Sigma_{h+1}, \ldots, \Sigma_{n_g})$}
\DP \\
\end{tabular}
\end{center}
\end{comment}

\begin{itemize}
\item Structural rules for lattice connectives:
\end{itemize}
\begin{center}
\begin{tabular}{rl}
\AX$\AATOP \fCenter \Delta$
\LL{\fns $\aatop_W$}
\UI$\Gamma \fCenter \Delta$
\DP
 & 
\AX$\Gamma \fCenter \ABOT$
\RL{\fns $\abot_W$}
\UI$\Gamma \fCenter \Delta$
\DP
\end{tabular}
\end{center}

\begin{itemize}
\item Logical introduction rules for lattice connectives:
\end{itemize}
\begin{center}
\begin{tabular}{rl}
\AX$\AATOP \fCenter \Delta$
\LL{\fns $\aatop_L$}
\UI$\aatop \fCenter \Delta$
\DP
 \ 
\AXC{$\phantom{\AATOP \fCenter \Delta}$}
\RL{\fns $\aatop_R$}
\UI$\AATOP \fCenter \aatop$
\DP
 & 
\AXC{$\phantom{\Gamma \fCenter \ABOT}$}
\LL{\fns $\abot_L$}
\UI$\abot \fCenter \ABOT$
\DP
 \ 
\AX$\Gamma \fCenter \ABOT$
\RL{\fns $\abot_R$}
\UI$\Gamma \fCenter \abot$
\DP
 \\

 & \\

\AX$\psi \fCenter \Delta$
\LL{\fns $\aand_{L2}$}
\UI$\varphi \aand \psi \fCenter \Delta$
\DP
 \ 
\AX$\varphi \fCenter \Delta$
\LL{\fns $\aand_{L1}$}
\UI$\varphi \aand \psi \fCenter \Delta$
\DP
 & 
\AX$\Gamma \fCenter \varphi$
\AX$\Gamma \fCenter \psi$
\RL{\fns $\aand_R$}
\BI$\Gamma \fCenter \varphi \aand \psi$
\DP
 \\

 & \\

\AX$\varphi \fCenter \Delta$
\AX$\psi \fCenter \Delta$
\LL{\fns $\aor_L$}
\BI$\varphi \aor \psi \fCenter \Delta$
\DP
 & 
\AX$\Gamma \fCenter \varphi$
\RL{\fns $\aor_{R1}$}
\UI$\Gamma \fCenter \varphi \aor \psi$
\DP
 \ 
\AX$\Gamma \fCenter \psi$
\RL{\fns $\aor_{R2}$}
\UI$\Gamma \fCenter \varphi \aor \psi$
\DP
 \\
\end{tabular}

\end{center}
%

\begin{itemize}
\item Logical introduction rules for $f\in\mathcal{F}$ and $g\in\mathcal{G}$:
\end{itemize}
				\begin{center}
					\begin{tabular}{c c}
						\bottomAlignProof
						\AX$\FH\, (\ophi) \fCenter \Delta$
						\LL{\fns$f_L$}
						\UI$f(\ophi) \fCenter \Delta$
						\DP
						&
						\bottomAlignProof
						\AX$\Gamma \fCenter \GC\, (\ophi)$
						\RL{\fns$g_R$}
						\UI$\Gamma \fCenter g(\ophi)$
						\DP
					\end{tabular}
					\begin{tabular}{c}
						\bottomAlignProof
						\AxiomC{$\Big(\Gamma_i \fCenter \varphi_i \quad \psi_j \fCenter \Delta_j \mid 1\leq i, j\leq n_f, \varepsilon_{f,i} = 1\mbox{ and } \varepsilon_{f,j} = \partial\Big)$}
						\RL{\fns$f_R$}
						\UI$\FH\, (\OSI)\fCenter f(\ophi)$
						\DP
					\end{tabular}
					\begin{tabular}{c c c }
						\bottomAlignProof
						\AxiomC{$\Big(\varphi_i \fCenter \Delta_i \quad \Gamma_j \fCenter \psi_j \,\mid\, 1\leq i, j\leq n_g, \varepsilon_{g,i} = 1\mbox{ and } \varepsilon_{g,j} = \partial \Big)$}
						\LL{\fns$g_L$}
						\UI$g(\ophi) \fCenter \GC\, (\OSI)$
						\DP
					\end{tabular}
				\end{center}
				%where $i$-monotone ($j$-antitone) means that the operator is order preserving (order reversing) at the $i$-th ($j$-th) coordinate.
				In particular, if $f$ and $g$ are $0$-ary (i.e.~they are constants), the rules $f_R$ and $g_L$ above reduce to the axioms ($0$-ary rules) $\FH \fCenter f$ and $g \fCenter \GC$.
	\iffalse			
\begin{itemize}
\item Only for $\mathrm{D.LE}^*$, introduction rules for each $f_i^\sharp, g_h^\flat\in (\mathcal{F}^*\cup\mathcal{G}^*)\setminus (\mathcal{F}\cup \mathcal{G})$:
\end{itemize}
				\begin{itemize}
					\item[] If $\varepsilon_{f,i} = 1$ and $\varepsilon_{g,h} = 1$,
				\end{itemize}
					\begin{center}
						\begin{tabular}{c c}
							\bottomAlignProof
							\AX$\GHF_h\, (\ophi, \opsi) \fCenter \Delta$
							\LL{\fns${g_h^\flat}_L$}
							\UI$g_h^\flat(\ophi, \opsi) \fCenter \Delta$
							\DP
							&
							\bottomAlignProof
							\AX$\Gamma \fCenter \FCS_i\, (\ophi, \opsi)$
							\RL{\fns${f_i^\sharp}_R$}
							\UI$\Gamma \fCenter f_i^\sharp(\ophi, \opsi)$
							\DP
						\end{tabular}
						\begin{tabular}{c}
							\bottomAlignProof
							\bottomAlignProof
							\AxiomC{$\Big(\Gamma_{\ell} \fCenter \varphi_{\ell} \quad \varphi_m \fCenter \Delta_m \mid 1\leq \ell, m\leq n_g, \varepsilon_{g_h^\flat, \ell} = 1\mbox{ and } \varepsilon_{g_h^\flat, m} = \partial \Big)$}
							\RL{\fns${g_h^\flat}_R$}
							\UI$\GHF_h\, (\OGA, \ODE) \fCenter g_h^\flat(\ophi, \opsi)$
							\DP
						\end{tabular}
						\begin{tabular}{c c c }
							\bottomAlignProof
							\AxiomC{$\Big( \varphi_\ell \fCenter \Delta_\ell \quad \Gamma_m \fCenter \varphi_m \,\mid\, 1\leq \ell, m\leq n_g, \varepsilon_{f_i^\sharp, \ell} = 1\mbox{ and } \varepsilon_{f_i^\sharp, m} = \partial \Big)$}
							\LL{\fns${f_i^\sharp}_L$}
							\UI$f_i^\sharp(\ophi, \opsi) \fCenter \FCS_i\, (\OGA, \ODE)$
							\DP
						\end{tabular}
					\end{center}
					%where $i$-monotone ($j$-antitone) means that the operator is order preserving (order reversing) at the $i$-th ($j$-th) coordinate.
					%In particular, if $f$ and $g$ are $0$-ary (i.e.\ they are constants), the rules above reduce to the axioms ($0$-ary rule) $H\fCenter f$ and $g\fCenter K$.
					\begin{itemize}
					\item[] If $\varepsilon_{f,i} = \partial$ and $\varepsilon_{g,h} = \partial$,
					\end{itemize}
					\begin{center}
						\begin{tabular}{c c}
							\bottomAlignProof
							\AX$\FHS_i\, (\ophi, \opsi) \fCenter \Delta$
							\LL{\fns${f_i^\sharp}_L$}
							\UI$f_i^\sharp(\ophi, \opsi) \fCenter \Delta$
							\DP
							&
							\bottomAlignProof
							\AX$\Gamma \fCenter \GCF_h\, (\ophi, \opsi)$
							\RL{\fns${g_h^\flat}_R$}
							\UI$\Gamma \fCenter g_h^\flat(\ophi, \opsi)$
							\DP
						\end{tabular}
						\begin{tabular}{c}
							\bottomAlignProof
							\bottomAlignProof
							\AxiomC{$\Big(\Gamma_{\ell} \fCenter \varphi_{\ell} \quad \varphi_m \fCenter \Delta_m \mid 1\leq \ell, m\leq n_f, \varepsilon_{f_i^\sharp, \ell} = 1\mbox{ and } \varepsilon_{f_i^\sharp, m} = \partial \Big)$}
							\RL{\fns${f_i^\sharp}_R$}
							\UI$\FHS_i\, (\OGA, \ODE) \fCenter f_i^\sharp(\ophi, \opsi)$
							\DP
						\end{tabular}
						\begin{tabular}{c c c }
							\bottomAlignProof
							\AxiomC{$\Big( \varphi_\ell \fCenter \Delta_\ell \quad \Gamma_m \fCenter \varphi_m \,\mid\, 1\leq \ell, m\leq n_g, \varepsilon_{g_h^\flat, \ell} = 1\mbox{ and } \varepsilon_{g_h^\flat, m} = \partial \Big)$}
							\LL{\fns${g_h^\flat}_L$}
							\UI$g_h^\flat(\ophi, \opsi) \fCenter \GCF_h\, (\OGA, \ODE)$
							\DP
						\end{tabular}
					\end{center}
\fi
% \item Introduction rules for additional connectives:
%  \begin{displaymath}
%\mathrm{(f_L)}\ \frac{\FH (\overline{\varphi})\Rightarrow y}{f(\overline{\varphi})\Rightarrow y} \quad \mathrm{(f_R)}\ \frac{\Big(x^{\epsilon_{f,i}} \Rightarrow \varphi_i \quad \varphi_j \Rightarrow x^{\epsilon_{f,j}}  \mid 1\leq i, j\leq n_f, \varepsilon_{f,i} = 1\mbox{ and } \varepsilon_{f,j} = \partial \Big)}{\FH(\overline{x})\Rightarrow f(\overline{\varphi})}
%\end{displaymath}
% \begin{displaymath}
%\mathrm{(g_L)}\ \frac{x \Rightarrow \GC(\overline{\psi})}{x \Rightarrow g(\overline{\psi})} \quad \mathrm{(g_R)}\ \frac{\Big( \psi_i \Rightarrow y^{\epsilon_{g,i}}  \quad y^{\epsilon_{g,j}}  \Rightarrow \psi_j \,\mid\, 1\leq i, j\leq n_g, \varepsilon_{g,i} = 1\mbox{ and } \varepsilon_{g,j} = \partial \Big)}{g(\overline{\psi}) \Rightarrow \GC (\overline{y})}		
%\end{displaymath}	



Let $\mathrm{cfD.LE}$ (resp.~$\mathrm{cfD.LE}$) denote the calculus obtained by removing Cut in $\mathrm{D.LE}$. In what follows, we indicate that the sequent $\varphi \Rightarrow \psi$ is derivable in $\mathrm{D.LE}$ (resp.~in $\mathrm{cfD.LE}$) by $\vdash_{\mathrm{D.LE}} \varphi \Rightarrow \psi$ (resp.~by $\vdash_{\mathrm{cfD.LE}} \varphi \Rightarrow \psi$).

\marginnote{AP: I think we should add a remark about the fact that the calculus is sound, complete and  conservative, and explain why}
\begin{prop}[Soundness]\label{prop:soundness of D.LE}
The calculus $\mathrm{D.LE}$ (and hence also $\mathrm{cfD.LE}$) is sound with respect to the class of  complete $\mathcal{L}$-algebras.
\end{prop}
\begin{proof}
The soundness of the basic lattice framework is clear. The soundness of the remaining rules uses the monotonicity (resp.~antitonicity) of the algebraic connectives interpreting each $f\in \mathcal{F}$ and $g\in \mathcal{G}$, and their adjunction/residuation properties, which hold since any complete $\mathcal{L}$-algebra is an $\mathcal{L}^*$-algebra.
\end{proof}

In the presentation of the language of the calculus above we use $\Gamma_1, \Gamma_2, \ldots$ and $\Delta_1, \Delta_2, \ldots$ as metavariables for structures. To formally present analytic structural rules, we need to utilize meta-strucutres, structures that are constructed by structural metavariables. In what follows, we will introduce explicitly a language of meta-variables and meta-terms, which will be useful in the remainder of this paper. Let $\mathsf{MVar} = \mathsf{MVar}_{\mathcal{F}}\uplus \mathsf{MVar}_{\mathcal{G}}$ be the denumerable set of {\em meta-variables} of sorts $\Gamma_1, \Gamma_2, \ldots\in \mathsf{MVar}_{\mathcal{F}}$ and $\Delta_1, \Delta_2, \ldots \in \mathsf{MVar}_{\mathcal{G}}$.
The sets $\mathsf{MStr}_\mathcal{F}$ and $\mathsf{MStr}_\mathcal{G}$ of the $\mathcal{F}$- and $\mathcal{G}$-{\em metastructures} are defined by simultaneous induction as follows:

\begin{center}
\begin{tabular}{rl}
$\mathsf{MStr}_\mathcal{F} \ni S$&$ ::= \Gamma \mid \FH(\overline{S})$\\

$\mathsf{MStr}_\mathcal{G} \ni T$&$ ::= \Delta \mid \GC(\overline{T})$
\end{tabular}
\end{center}
where $\FH \in \mathcal{F}^\ast$ and $\GC \in \mathcal{G}^\ast$ and $\overline{S} \in \mathsf{MStr}_\mathcal{F}^{\epsilon_f}$,  and $\overline{T} \in \mathsf{MStr}_\mathcal{G}^{\epsilon_g}$, and for any order type $\epsilon$ on $n$, we let $\mathsf{MStr}_\mathcal{F}^{\epsilon} : = \prod_{i = 1}^{n}\mathsf{MStr}_\mathcal{F}^{\epsilon(i)}$ and $\mathsf{MStr}_\mathcal{G}^{\epsilon} : = \prod_{i = 1}^{n}\mathsf{MStr}_\mathcal{G}^{\epsilon(i)}$, where for all $1 \leq i \leq n$,

\begin{center}
\begin{tabular}{ll}
$\mathsf{MStr}_\mathcal{F}^{\epsilon(i)} = \begin{cases} 
\mathsf{MStr}_\mathcal{F} &\mbox{ if } \epsilon(i) = 1\\
\mathsf{MStr}_\mathcal{G} &\mbox{ if } \epsilon(i) = \partial
\end{cases}\quad$
&
$\mathsf{MStr}_\mathcal{G}^{\epsilon(i)} = \begin{cases}
\mathsf{MStr}_\mathcal{G}& \mbox{ if } \epsilon(i) = 1,\\
\mathsf{MStr}_\mathcal{F} & \mbox{ if } \epsilon(i) = \partial.
\end{cases}$
\end{tabular}
\end{center}

An analytic structural rule is formally represented by a rule of the form
\begin{center}
\AXC{$(S_1\Rightarrow T_1)[\OSI_1]$}
\AXC{$\cdots$}
\AXC{$(S_n\Rightarrow T_n)[\OSI_n]$}
\TIC{$(S_0 \Rightarrow T_0)[\OSI_0]$}
\DP
\end{center}
where $\OSI_i$ with $0 \leq i \leq n$ is the set of metavariables occurring in each sequent $S_i \Rightarrow T_i$, $\OSI_0 \supseteq \OSI_1 \cup \ldots \cup \OSI_n$, and while structural metavariables might occur multiple times in the premises they occur only once in the conclusion. %Furthermore, we say that the rule maintains the subformula property, if every structural metavariable that appears in the sequents $S_1\Rightarrow T_1,\ldots S_n\Rightarrow T_n$ appears also in the conclusion $S_0\Rightarrow T_0$. 
An instance of the rule $R$ is obtained from $R$ by uniformly substituting each structural meta-variable $\Gamma\in \mathsf{MVar}_{\mathcal{F}}$ with an element of $\mathsf{Str}_{\mathcal{F}}$ and every structural metavariable $\Delta\in \mathsf{MVar}_{\mathcal{G}}$ with an element of $\mathsf{Str}_{\mathcal{G}}$. A calculus $\mathcal{D}$ contains the analytic rule $R$ if it contains every instance of $R$.
%In what follows, let $(\Gamma\Rightarrow \Delta)[\overline{\gamma}, \overline{\delta}]$ denote a D.LE-sequent, in which the vector $\overline{\gamma}$ (resp.~$\overline{\delta}$)  includes the  variables in $\mathsf{AtomStr}_\mathcal{F}$(resp.~$\mathsf{AtomStr}_\mathcal{G}$)  occurring in $\Gamma$ or in $\Delta$. A {\em structural rule} of D.LE is of the following form: 
%\begin{center}
%\AXC{$(\Gamma_1\Rightarrow \Delta_1)[\overline{\gamma}, \overline{\delta}]$}
%\AXC{$\cdots$}
%\AXC{$(\Gamma_n\Rightarrow \Delta_n)[\overline{\gamma}, \overline{\delta}]$}
%\TIC{$(\Gamma \Rightarrow \Delta)[\overline{\gamma}, \overline{\delta}]$}
%\DP
%\end{center}
%such that each $\gamma$ in $\overline{\gamma}$ (resp.~$\delta$ in  $\overline{\delta}$) is {\em parametric} (cf.~\cite{}).\marginnote{AP: do we have the def of parametric? can we cite or refer to something?} Such a structural rule is {\em analytic} if  each $\gamma$ in $\overline{\gamma}$ (resp.~$\delta$ in  $\overline{\delta}$) occurring in some premise of the rule also occurs in its conclusion, in which case, it occurs in the conclusion exactly once.

%In what follows, we will need to talk about structural rules, and their shape, as they are given in a display calculus. 
\begin{example}
 Given the LE-language $\mathcal{L}_\mathrm{LE}(\{\mand\},\{\wbox,\backslash\})$ considered in Example \ref{ex:1}, the following is an analytic structural rule: 
\begin{center}
\AX$\Gamma_1 \fCenter (\Gamma_2 \MAND \Gamma_3) \MRARR \WBOX\Delta$
\UI$\Gamma_1 \MAND \BDIA\Gamma_2 \fCenter \Delta \MLARR  \Gamma_3$
\DP
\end{center}
This rule is such that $\Gamma_1, \Gamma_2$, $\Gamma_3$ and $\Delta$ are metavariables which range over $\mathsf{Str}_{\mathcal{F}}$, and $\mathsf{Str}_{\mathcal{G}}$ respectively, and $(\Gamma_2 \MAND \Gamma_3) \MRARR \WBOX\Delta$, $\Gamma_1 \MAND \BDIA\Gamma_2$ and $\Delta \MLARR  \Gamma_3$ are metaterms. 
\end{example}





